Gerrymandering on graphs: Computational complexity and parameterized algorithms

Partitioning a region into districts to favor a particular candidate or a party is commonly known as gerrymandering. In this paper, we investigate the gerrymandering problem in graph theoretic setting as proposed by Cohen-Zemach et al. [AAMAS 2018]. Our contributions in this article are two-fold, conceptual and computational. We first resolve the open question posed by Ito et al. [AAMAS 2019] about the computational complexity of the problem when the input graph is a path. Next, we propose a generalization of their model, where the input consists of a graph on $n$ vertices representing the set of voters, a set of $m$ candidates $\mathcal{C}$, a weight function $w_v: \mathcal{C}\rightarrow {\mathbb Z}^+$ for each voter $v\in V(G)$ representing the preference of the voter over the candidates, a distinguished candidate $p\in \mathcal{C}$, and a positive integer $k$. The objective is to decide if one can partition the vertex set into $k$ pairwise disjoint connected sets (districts) s.t $p$ wins more districts than any other candidate. The problem is known to be NPC even if $k=2$, $m=2$, and $G$ is either a complete bipartite graph (in fact $K_{2,n}$) or a complete graph. This means that in search for FPT algorithms we need to either focus on the parameter $n$, or subclasses of forest. Circumventing these intractable results, we give a deterministic and a randomized algorithms for the problem on paths running in times $2.619^{k}(n+m)^{O(1)}$ and $2^{k}(n+m)^{O(1)}$, respectively. Additionally, we prove that the problem on general graphs is solvable in time $2^n (n+m)^{O(1)}$. Our algorithmic results use sophisticated technical tools such as representative set family and Fast Fourier transform based polynomial multiplication, and their (possibly first) application to problems arising in social choice theory and/or game theory may be of independent interest to the community.

==> abstract-old.tex <==
% !TEX root = main.tex

The practice of partitioning a region into areas to favor a particular candidate or a party in an election has been known to exist for the last two centuries. This practice is commonly known as {\em gerrymandering}. In this paper, we continue investigating the gerrymandering problem in the graph theoretic setting as proposed by Cohen-Zemach et al. [AAMAS 2018] and continued by Ito et al. [AAMAS 2019].  Our contributions in this article are two-fold, conceptual and computational. We first resolve the open question posed by Ito et al. [AAMAS 2019] about the computational complexity of gerrymandering when the graph is a path. Next, we propose a generalization of the model studied in [AAMAS 2019], where the input consists of a graph on $n$ vertices representing the set of voters, a set of $m$ candidates $\mathcal{C}$, a weight function $w_v: \mathcal{C}\rightarrow {\mathbb Z}^+$ for each voter $v\in V(G)$ representing the preference of the voter over the candidates, a distinguished candidate $p\in \mathcal{C}$, and a positive integer $k$. %\hide{In [AAMAS 2019], $w_{v}(c) \neq 0$ for a unique candidate, but we allow the function to be arbitrary.} 
The objective is to decide if it is possible to partition the vertex set into $k$ {\it districts} (i.e., pairwise disjoint connected sets) such that the candidate $p$ {\em wins} more districts than any other candidate. We show that the problem admits a $2^n (n+m)^{\mathcal{O}(1)}$ time algorithm. Furthermore, we  complement the intractability result for path by a parameterized algorithm with respect to the parameter $k$ in both deterministic and randomized settings, even for arbitrary weight functions. \Ma{Our algorithmic results use deep technical tools such as representative set family and Fast Fourier transform based polynomial multiplication, and their (possibly first) application to problems arising in social choice theory and/or algebraic game theory may be of independent interest to the community.} \ma{Add this? }






%an arbitrary weight function $w_{v}$. 
%Since the problem is Complementing the intractability result shown above, we show that even the weighted version of the problem is tractable from the perspective of parameterized complexity, whereby the problem is {\it fixed parameter tractable} with respect to the parameter $k$ in both deterministic and randomized settings, even for an arbitrary weight function $w_{v}$. Moreover, 




%\begin{supress}
%\il{OLD-AAMAS version}
%
%The practice of partitioning a region into areas to favor a particular candidate or a party in an election has been known to exist for the last two centuries. This practice is commonly known as {\em gerrymandering}. In this paper we continue investigating the gerrymandering problem in the graph theoretic setting as proposed by Cohen-Zemach et. al \cite{ZemachLR18} and continued by Ito et al.~[AAMAS 2019].  Our contributions in this article are two-fold, conceptual and computational. We propose a generalization of the model studied in [AAMAS 2019], where the input consists of a graph on $n$ vertices representing the set of voters, a set of $m$ candidates \mathcal{C}, a weight function $w_v: \mathcal{C}\rightarrow {\mathbb Z}^+$ for each voter $v\in V(G)$ representing the preference of the voter over the candidates, a distinguished candidate $p\in \mathcal{C}$, and a positive integer $k$.\hide{In [AAMAS 2019], $w_{v}(c) \neq 0$ for a unique candidate, but we allow the function to be arbitrary.} The objective is to decide if it is possible to partition the vertex set into $k$ {\it districts} (i.e pairwise disjoint connected sets) such that the candidate $p$ {\em wins} more districts than any other candidate. We resolve an open question posed by Ito et al. [AAMAS 2019] about the computational complexity of the special case of the above problem when the graph is a path and the voter's weight function $w_{v}$, for any $v\in V(G)$, gives a non-zero value to a single candidate only. Complementing this classical intractability result, we show that in fact, this problem is tractable from the perspective of parameterized complexity, whereby the problem is {\it fixed parameter tractable} with respect to the parameter $k$ in both deterministic and randomized settings, even for an arbitrary weight function $w_{v}$. Moreover, we show that on general graphs the problem admits a $2^n (n+m)^{\mathcal(1)}$ time algorithm. %\Ma{Our algorithmic techniques use representative family and algebraic techniques.}
%\end{supress}
%
%
%\begin{supress}
%\il{OLD}
%
%Formally, in the weighted gerrymandering problem over graphs, the input is a set of $n$ voters, represented by the vertices in a graph, a set of $m$ candidates \mathcal{C}, a weight function $w_v \mathcallon \mathcal{C}\rightarrow {\mathbb Z}^+$ for each voter $v$ representing the preference of the voter over the candidates, a distinguished candidate $p\in \mathcal{C}$, and a positive integer $k$. The objective is to decide if it is possible to create $k$ pairwise disjoint districts (a connected set of voters in the graph) containing all the voters such that the candidate $p$ {\em wins} more districts than any other candidate. In this paper, we study this problem from the lens of multivariate complexity and design several algorithms for different instantiations of the problem. We first prove that even when the input graph is a path this problem is \npc. Complementing this negative result, we give 
%% Furthermore, we study the problem from the perspective of parameterized and exact exponential time algorithms. We prove that there are
%a deterministic and a randomized algorithms for the problem on paths running in times $2.619^{k}(n+m)^{\mathcal(1)}$ and $2^{k}(n+m)^{\mathcal(1)}$, respectively. Additionally, we prove that the problem on general graphs is solvable in time $2^n (n+m)^{\mathcal(1)}$.
%\end{supress}
 
